Complex Valued Gated Auto-encoder for Video Frame Prediction

In recent years, complex valued artificial neural networks have gained increasing interest as they allow neural networks to learn richer representations while potentially incorporating less parameters. Especially in the domain of computer graphics, many traditional operations rely heavily on computations in the complex domain, thus complex valued neural networks apply naturally. In this paper, we perform frame predictions in video sequences using a complex valued gated auto-encoder. First, our method is motivated showing how the Fourier transform can be seen as the basis for translational operations. Then, we present how a complex neural network can learn such transformations and compare its performance and parameter efficiency to a real-valued gated autoencoder. Furthermore, we show how extending both - the real and the complex valued - neural networks by using convolutional units can significantly improve prediction performance and parameter efficiency. The networks are assessed on a moving noise and a bouncing ball dataset.

==> sections/PGP_method.tex <==
\section{Complex Valued Predictive Gating Pyramid}

\subsection{Gated Auto-Encoders}
In this section, we want to briefly discuss the mathematical concepts behind Gated Auto-Encoders, as described by Memisevic \cite{memisevic2013learning} (in the following referred as "real valued GAE") and Gated Auto-Encoders with tied input weights, as described by Droniou et Al. \cite{droniou2013gated} (in the following referred as "complex valued GAE") as they build the foundation for the predictive gating pyramid (PGP) \cite{michalski2014modeling} as well as our proposed complex valued PGP architecture. Let us assume, the transformation between two images at time at time points $t$ and $t-1$ is linear, then:
\begin{equation}
    X_t = L X_{t-1}
\label{eq:1}
\end{equation}
Here, $X_t$ and $X_{t-1}$ denote the vectorized form of the two images and $L$ denotes a transformation matrix.
If we further assume, that the transformation is orthogonal, $L$ can be decomposed into:
\begin{equation}
    L = UDU^*
\label{eq:2}
\end{equation}
with U being a unitary matrix ($UU^*=I$) and D being a diagonal matrix containing complex numbers of absolute value 1. While the assumption of a linear orthogonal transformation at first glance seems quite restricting it still comprises for example all transformations that can be described as pixel permutations (e.g. translation/rotation/shearing). From \ref{eq:1} and \ref{eq:2}, it follows that:
\begin{equation}
    U^*X_t = D U^* X_{t-1} \Rightarrow D = \mathop{\mathrm{diag}}\left( \frac{U^* X_t}{U^*X_{t-1}}\right)
\label{eq:3}
\end{equation}
This is remarkable since it shows how orthogonal linear transformations can be represented in a much more compact way as rotations in the complex plane by $D$ when the basis is properly changed by $U$. If we consider for example only translational transformations, $U^*$ basically becomes a discrete fourier transform and $D$ corresponds to phase-shifts in frequency domain. The obtained representation of the transformation can be used to extrapolate to future images:
\begin{equation}
    X_{t+k} = U D^k U^* X_t
\label{eq:4}
\end{equation}
This however leads to problems when projections of $U$ lead to small absolute values, because in this case the computation of $D$ becomes unstable resulting in falsely detected transformations.

Thus Memisevic \cite{memisevic2013learning} --- inspired by these theoretical foundations --- constructed a trainable bi-linear model; the real valued GAE. In this architecture, several trainable linear modules $U,U',V,V'$ learn representations of $U^*$ and phase-shifted representations of $U^*$ respectively. The weights in between $U,U'$ and $V,V'$ are shared. Furthermore, in order to properly normalize the representation of the transformation, two additional linear modules ($W$ and $W'^T$) together with a sigmoid-nonlinearity are used. During our experiments we investigated fully connected as well as convolutional units inside these linear modules. After having obtained the relational features ($m$), they are either multiplied ("gated") by $U' X_{t-1}$ in the case of reconstruction or by $U' X_t$ in the case of prediction and projected back by $V'^T$:
\begin{align}
    m &= \sigma(W(U X_{t-1}\cdot V X_t)) &\mathrm{relational\ features}\\
    X_t &= V'^T (U'X_{t-1} \cdot W'^T m) &\mathrm{reconstruction}\\
    X_{t+1} &= V'^T (U'X_t \cdot W'^T m) &\mathrm{prediction}
\end{align}
While this real valued GAE is able to learn robust relational features for a wide range of linear transformations, Droniou et Al. \cite{droniou2013gated} later pointed out that parameter efficiency can be drastically increased since $U$ and $V$ learn mostly the same features. They suggested a complex valued GAE, which directly makes use of equation \ref{eq:3}. By treating $U^*$ in the complex domain, it is not further needed to learn $U$ and $V$ separately. Instead, by carefully designing the matrices $E_1,E_2,E_3,P,R$ (see \cite{droniou2013gated} for exact definitions), the network is able to perform all computations directly in complex domain and thus is able to spare out $V$ (see also Figure \ref{model_architectures} c) for a schematic depiction). This not only results in fewer parameters but also in a strong prior potentially speeding up convergence. While Droniou et Al. showed, how complex valued GAE can be used for reconstruction (see equation \ref{Droniou_reconstruction}) we were able to evidence that it is as capable for prediction:

\begin{align}
    m &= \sigma(W P (E_1 U^T X_{t-1}\cdot E_2 U'^T X_t)) &\mathrm{relational\ features}\\
    X_t &= U'' R P (E_1 U'^T X_{t-1} \cdot E_3 W'^T m) &\mathrm{reconstruction}\label{Droniou_reconstruction}\\
    X_{t+1} &= U'' R P (E_1 U'^T X_t \cdot E_3 W'^T m) &\mathrm{prediction}
\end{align}

Since GAE scale quadratic in the number of image pixels, we also propose a convolutional form of the real and complex valued GAE which replaces the originally fully connected modules $U,V,W$ by convolutional units. The matrices $E_1,E_2,E_3,P$ for the complex valued GAE also stay the same but now are applied on the corresponding channels.

\subsection{Predictive Gating Pyramid}
The predictive gating pyramid is an architecture proposed by Michalski et Al. \cite{michalski2014modeling} to predict video frames by using a 



==> sections/related.tex <==
\section{Related Work}
\label{related}

Different methods have been proposed to solve the task of video prediction and the most successful ones are based on the \ac{DNN} architectures.  \citet{michalski2014modeling} designed a recurrent network to predict the next future frames by  proposing a bi-linear model of transformations which were applied to pairs of frames $(\text{frame}_{t-1}, \text{frame}_{t}) $ to predict $\text{frame}_{t+1}$.  \citet{demodeling} proposed its equivalent fully convolutional form which reduced the number of parameters in the order of magnitude and less training time. The \ac{PGP} architecture is designed based on the \ac{GAE} architecture, which was improved and analyzed by \citet{droniou2013gated} in the complex domain. The results represent that with the half number of parameters of the \ac{GAE} architecture, they got same result. 

%complex cnn related work
